Feasibility of Detecting Cognitive Impairment and Psychological Well-being among Older Adults Using Facial, Acoustic, Linguistic, and Cardiovascular Patterns Derived from Remote Conversations

The aging society urgently requires scalable methods to monitor cognitive decline and identify social and psychological factors indicative of dementia risk in older adults. Our machine learning (ML) models captured facial, acoustic, linguistic, and cardiovascular features from 39 older adults with normal cognition or Mild Cognitive Impairment (MCI), derived from remote video conversations and quantified their cognitive status, social isolation, neuroticism, and psychological well-being. Our model could distinguish Clinical Dementia Rating Scale (CDR) of 0.5 (vs. 0) with 0.77 area under the receiver operating characteristic curve (AUC), social isolation with 0.74 AUC, social satisfaction with 0.75 AUC, psychological well-being with 0.72 AUC, and negative affect with 0.74 AUC. Our feature importance analysis showed that speech and language patterns were useful for quantifying cognitive impairment, whereas facial expressions and cardiovascular patterns were useful for quantifying social and psychological well-being. Our bias analysis showed that the best-performing models for quantifying psychological well-being and cognitive states in older adults exhibited significant biases concerning their age, sex, disease condition, and education levels. Our comprehensive analysis shows the feasibility of monitoring the cognitive and psychological health of older adults, as well as the need for collecting largescale interview datasets of older adults to benefit from the latest advances in deep learning technologies to develop generalizable models across older adults with diverse demographic backgrounds and disease conditions.

==> markup.tex <==
% =========================
% Markup helpers for text, figures, and tables
% Versions: og | mp | fi
%   og = original (show removed, hide new)
%   mp = marked-up (red strikeouts, blue additions, blue boxes/X on floats)
%   fi = final (show new as normal, hide removed)
% =========================

\providecommand{\docversion}{mp} % <-- override in MAIN with \renewcommand{\docversion}{...}

% ---------- Packages ----------
\usepackage{ifthen}
\usepackage[normalem]{ulem}   % \sout
\usepackage{xcolor}
\usepackage{comment}
\usepackage[most]{tcolorbox}
\usepackage{tikz}
\usepackage{currfile}         % \currfilename
\usepackage{zref-abspage}     % absolute page refs for logging
\usepackage{lineno}           % optional visible line numbers in mp

% Optional visible line numbers in marked-up mode:
\ifthenelse{\equal{\docversion}{mp}}{\linenumbers}{}

% ---------- Change log (CSV) ----------
% Writes one CSV per run: <jobname>-changes.csv
% columns: category,action,content,file,line,abspage
\newwrite\changelog
\immediate\openout\changelog=\jobname-changes.csv
\immediate\write\changelog{category,action,content,file,line,abspage}
\AtEndDocument{\immediate\closeout\changelog}

\makeatletter
\newcommand{\LogChange}[3]{% #1=category(text/figure/table), #2=action(add/remove), #3=content
  \begingroup
    % label to capture absolute page on second run
    \zref@labelbyprops{chg@\the\year @\the\time @\the\inputlineno}{abspage}%
    \edef\thispage{\zref@extractdefault{chg@\the\year @\the\time @\the\inputlineno}{abspage}{0}}%
    \edef\thisfile{\currfilename}%
    % crude CSV-safe content
    \edef\safecontent{\detokenize{#3}}%
    \immediate\write\changelog{#1,#2," \safecontent ",\thisfile,\the\inputlineno,\thispage}%
  \endgroup
}
\makeatother

% ---------- Text markup ----------
\DeclareRobustCommand{\removed}[1]{%
  \ifthenelse{\equal{\docversion}{mp}}{%
    \textcolor{red}{\sout{#1}}%
    \LogChange{text}{remove}{#1}%
  }{%
    \ifthenelse{\equal{\docversion}{og}}{%
      #1\unskip % show in "original"
    }{%
      \ignorespaces % hide in "final"
    }%
  }%
}

\DeclareRobustCommand{\new}[1]{%
  \ifthenelse{\equal{\docversion}{mp}}{%
    \textcolor{blue}{#1}%
    \LogChange{text}{add}{#1}%
  }{%
    \ifthenelse{\equal{\docversion}{fi}}{%
      #1\unskip % show as normal in "final"
    }{%
      \ignorespaces % hide in "original"
    }%
  }%
}
% (Optional alias if you prefer an unambiguous name)
\DeclareRobustCommand{\addedtext}[1]{\new{#1}}

% ---------- Figure/Table wrappers ----------
% Use these instead of plain figure/table when adding/removing floats.
% They ensure proper begin/end matching and log via \caption{...} text.

% --- ADDED FIGURE ---
% \newenvironment{addedfigure}[1][tbp]{%
%   \begin{figure}[#1]%
%   \ifthenelse{\equal{\docversion}{og}}{%
%     \begin{comment}%
%   }{%
%     \begingroup
%     \let\origcaption\caption
%     \renewcommand{\caption}[1]{\origcaption{##1}\LogChange{figure}{add}{##1}}%
%     \ifthenelse{\equal{\docversion}{mp}}{%
%       \begin{tcolorbox}[enhanced,breakable,boxrule=1pt,colframe=blue]%
%     }{}%
%   }%
% }{%
%   \ifthenelse{\equal{\docversion}{og}}{%
%     \end{comment}%
%   }{%
%     \ifthenelse{\equal{\docversion}{mp}}{\end{tcolorbox}}{}%
%     \endgroup
%   }%
%   \end{figure}%
% }

% requires: \usepackage{ifthen,comment,tcolorbox}
% tcolorbox recommended options: \tcbset{enhanced}
\newenvironment{addedfigure}[1][tbp]{%
  \begin{figure}[#1]%
  \ifthenelse{\equal{\docversion}{og}}{%
    \begin{comment}%
  }{%
    \begingroup
    % keep your change logger
    \let\origcaption\caption
    \renewcommand{\caption}[1]{\origcaption{##1}\LogChange{figure}{add}{##1}}%
    % open a full-width, zero-padding box that will include image + caption
    \ifthenelse{\equal{\docversion}{mp}}{%
      \begin{tcolorbox}[
        enhanced,
        colframe=blue,
        colback=white,
        boxrule=1pt,
        sharp corners,
        width=\linewidth,
        left=0pt,right=0pt,top=0pt,bottom=0pt,
        boxsep=0pt,
        enlarge left by=0mm,
        enlarge right by=0mm
      ]%
      \begin{minipage}{\linewidth}%
    }{%
      \begin{minipage}{\linewidth}%
    }%
  }%
}{%
  \ifthenelse{\equal{\docversion}{og}}{%
    \end{comment}%
  }{%
      \end{minipage}%
      \ifthenelse{\equal{\docversion}{mp}}{\end{tcolorbox}}{}%
      \endgroup
  }%
  \end{figure}%
}


% --- REMOVED FIGURE ---
\newenvironment{removedfigure}[1][tbp]{%
  \begin{figure}[#1]%
  \ifthenelse{\equal{\docversion}{fi}}{%
    \begin{comment}%
  }{%
    \begingroup
    \let\origcaption\caption
    \renewcommand{\caption}[1]{\origcaption{##1}\LogChange{figure}{remove}{##1}}%
    \ifthenelse{\equal{\docversion}{mp}}{%
      \begin{tcolorbox}[enhanced,breakable,boxrule=1.25pt,colframe=red,
        overlay={\draw[red,line width=1.5pt] (frame.north west)--(frame.south east);
                 \draw[red,line width=1.5pt] (frame.north east)--(frame.south west);} ]%
    }{}%
  }%
}{%
  \ifthenelse{\equal{\docversion}{fi}}{%
    \end{comment}%
  }{%
    \ifthenelse{\equal{\docversion}{mp}}{\end{tcolorbox}}{}%
    \endgroup
  }%
  \end{figure}%
}

% --- ADDED TABLE ---
% \newenvironment{addedtable}[1][tbp]{%
%   \begin{table}[#1]%
%   \ifthenelse{\equal{\docversion}{og}}{%
%     \begin{comment}%
%   }{%
%     \begingroup
%     \let\origcaption\caption
%     \renewcommand{\caption}[1]{\origcaption{##1}\LogChange{table}{add}{##1}}%
%     \ifthenelse{\equal{\docversion}{mp}}{%
%       \begin{tcolorbox}[enhanced,breakable,boxrule=1pt,colframe=blue]%
%     }{}%
%   }%
% }{%
%   \ifthenelse{\equal{\docversion}{og}}{%
%     \end{comment}%
%   }{%
%     \ifthenelse{\equal{\docversion}{mp}}{\end{tcolorbox}}{}%
%     \endgroup
%   }%
%   \end{table}%
% }
% --- ADDED TABLE (no overlap) ---
\newenvironment{addedtable}[1][tbp]{%
  \begin{table}[#1]%
  \ifthenelse{\equal{\docversion}{og}}{%
    \begin{comment}%
  }{%
    \begingroup
    \let\origcaption\caption
    \renewcommand{\caption}[1]{\origcaption{##1}\LogChange{table}{add}{##1}}%
    % disable line numbers inside the float (lineno is fragile here)
    \ifthenelse{\equal{\docversion}{mp}}{\begin{nolinenumbers}}{}%
    % draw the blue frame, but keep the content as ONE solid box
    \ifthenelse{\equal{\docversion}{mp}}{%
      \begin{tcolorbox}[
        enhanced,
        colframe=blue,
        colback=white,
        boxrule=1pt,
        sharp corners,
        width=\linewidth,
        left=0pt,right=0pt,top=0pt,bottom=0pt,
        boxsep=0pt
      ]%
      \begin{minipage}{\linewidth}%
    }{%
      \begin{minipage}{\linewidth}%
    }%
  }%
}{%
  \ifthenelse{\equal{\docversion}{og}}{%
    \end{comment}%
  }{%
      \end{minipage}%
      \ifthenelse{\equal{\docversion}{mp}}{\end{tcolorbox}\end{nolinenumbers}}{}%
      \endgroup
  }%
  \end{table}%
}


% Preamble needs:
% \usepackage{environ,ifthen,tikz}
% \usetikzlibrary{calc}

\NewEnviron{removedtable}[1][tbp]{%
  \ifthenelse{\equal{\docversion}{fi}}%
    {}% final: omit entirely
    {%
      \begin{table}[#1]
        \centering
        \begin{tikzpicture}
          \node[inner sep=0,outer sep=0] (B) {%
            \begin{minipage}{\linewidth}
              \BODY
            \end{minipage}
          };
          \draw[red,line width=1.25pt] (B.north west) rectangle (B.south east);
          \draw[red,line width=1.25pt] (B.north west) -- (B.south east);
          \draw[red,line width=1.25pt] (B.north east) -- (B.south west);
        \end{tikzpicture}
      \end{table}%
    }%
}



% \makeatletter
% \NewEnviron{removedtable}[1][tbp]{%
%   \begin{table}[#1]%
%   \ifthenelse{\equal{\docversion}{fi}}{%
%     \begin{comment}%
%   }{%
%     % Box everything (caption + table) so height/width are known:
%     \begin{center}
%     \begin{tikzpicture}
%       \node[inner sep=0,outer sep=0] (B) {%
%         \begin{minipage}{\linewidth} % column width; use \textwidth for full-width floats
%           % Clamp any wide bodies to the column width:
%           \begin{adjustbox}{max width=\linewidth}
%             \begin{minipage}{\linewidth}
%               \BODY
%             \end{minipage}
%           \end{adjustbox}
%         \end{minipage}
%       };
%       % Red border + X fully around the content:
%       \draw[red, line width=1.25pt] (B.north west) rectangle (B.south east);
%       \draw[red, line width=1.25pt] (B.north west) -- (B.south east);
%       \draw[red, line width=1.25pt] (B.north east) -- (B.south west);
%     \end{tikzpicture}
%     \end{center}
%   }%
%   \ifthenelse{\equal{\docversion}{fi}}{\end{comment}}{}%
%   \end{table}%
% }
% \makeatother





% --- REMOVED TABLE ---
% \newenvironment{removedtable}[1][tbp]{%
%   \begin{table}[#1]%
%   \ifthenelse{\equal{\docversion}{fi}}{%
%     \begin{comment}%
%   }{%
%     \begingroup
%     \let\origcaption\caption
%     \renewcommand{\caption}[1]{\origcaption{##1}\LogChange{table}{remove}{##1}}%
%     \ifthenelse{\equal{\docversion}{mp}}{%
%       \begin{tcolorbox}[enhanced,breakable,boxrule=1.25pt,colframe=red,
%         overlay={\draw[red,line width=1.5pt] (frame.north west)--(frame.south east);
%                  \draw[red,line width=1.5pt] (frame.north east)--(frame.south west);} ]%
%     }{}%
%   }%
% }{%
%   \ifthenelse{\equal{\docversion}{fi}}{%
%     \end{comment}%
%   }{%
%     \ifthenelse{\equal{\docversion}{mp}}{\end{tcolorbox}}{}%
%     \endgroup
%   }%
%   \end{table}%
% }



